A physical model for the [CII]-FIR deficit in luminous galaxies

Observations of ionised carbon at 158 micron ([CII]) from luminous star-forming galaxies at z~0 show that their ratios of [CII] to far infrared (FIR) luminosity are systematically lower than those of more modestly star-forming galaxies. In this paper, we provide a theory for the origin of this so called "[CII] deficit" in galaxies. Our model treats the interstellar medium as a collection of clouds with radially-stratified chemical and thermal properties, which are dictated by the clouds' volume and surface densities, as well as the interstellar radiation and cosmic ray fields to which they are exposed. [CII] emission arises from the outer, HI dominated layers of clouds, and from regions where the hydrogen is H2 but the carbon is predominantly C+. In contrast, the most shielded regions of clouds are dominated by CO and produce little [CII] emission. This provides a natural mechanism to explain the observed [CII]-star formation relation: galaxies' star formation rates are largely driven by the surface densities of their clouds. As this rises, so does the fraction of gas in the CO-dominated phase that produces little [CII] emission. Our model further suggests that the apparent offset in the [CII]-FIR relation for high-z sources compared to those at present epoch may arise from systematically larger gas masses at early times: a galaxy with a large gas mass can sustain a high star formation rate even with relatively modest surface density, allowing copious [CII] emission to coexist with rapid star formation.

==> pdflatex.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{malhotra97a,luhman98a,nikola98a}
\citation{stacey91a}
\citation{goldsmith12a}
\citation{stacey91a}
\citation{leech99a}
\citation{boselli02a}
\citation{delooze11a,sargsyan12a,pineda14a,herreracamus15a}
\citation{olsen15a}
\newlabel{firstpage}{{}{1}{}{Doc-Start}{}}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}}
\newlabel{section:introduction}{{1}{1}{Introduction}{section.1}{}}
\citation{malhotra97a,malhotra01a,luhman98a,luhman03b}
\citation{graciacarpio11a}
\citation{diazsantos13a}
\citation{beirao12a}
\citation{croxall12a}
\citation{farrah13a}
\citation{casey14a}
\citation{iono06a,stacey10a,wagg12a,swinbank12a,rawle13a,riechers13a,wang13a,rigopoulou14a,brisbin15a}
\citation{krumholz08a,krumholz09a,mckee10a}
\citation{krumholz13a,krumholz13c}
\citation{krumholz08a,krumholz09a,krumholz09b}
\citation{mckee10a}
\@writefile{toc}{\contentsline {section}{\numberline {2}Model Description}{2}{section.2}}
\newlabel{section:model}{{2}{2}{Model Description}{section.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1}Cloud Physical Structure}{2}{subsection.2.1}}
\newlabel{ssec:phys_struct}{{2.1}{2}{Cloud Physical Structure}{subsection.2.1}{}}
\newlabel{equation:kmt}{{1}{2}{Cloud Physical Structure}{equation.1}{}}
\citation{bertoldi92a}
\citation{dobbs11a,dobbs13a,heyer15a}
\citation{krumholz11a,glover11a,krumholz12c}
\citation{krumholz07b,krumholz12a,krumholz14a}
\citation{dobbs14a,heyer15a}
\citation{kennicutt12a}
\citation{bigiel08a,blanc09a,narayanan11a,narayanan11b,narayanan12a,shetty13b,shetty13a}
\citation{narayanan12a}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Parameters used in cloud models  }}{3}{table.1}}
\newlabel{table:free_parameters}{{1}{3}{Parameters used in cloud models}{table.1}{}}
\newlabel{equation:mass}{{3}{3}{Cloud Physical Structure}{equation.3}{}}
\newlabel{eq:sigmac}{{6}{3}{Cloud Physical Structure}{equation.6}{}}
\newlabel{eq:sfr}{{7}{3}{Cloud Physical Structure}{equation.7}{}}
\newlabel{eq:tff}{{8}{3}{Cloud Physical Structure}{equation.8}{}}
\citation{wolfire03a}
\citation{heyer15a}
\citation{robitaille10a}
\citation{chomiuk11a}
\citation{bolatto08a,leroy13a}
\citation{saintonge11a,bothwell13a}
\citation{murphy11a}
\citation{kennicutt12a}
\citation{draine11a}
\citation{nelson99a}
\citation{glover07a}
\citation{glover07a}
\citation{glover12a}
\citation{glover12a}
\citation{glover12a}
\citation{glover12a}
\citation{robitaille10a,chomiuk11a}
\citation{glover12a}
\citation{draine96a}
\citation{vandishoeck88a}
\newlabel{eq:rhoscaling}{{9}{4}{Cloud Physical Structure}{equation.9}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2}Chemical Structure}{4}{subsection.2.2}}
\newlabel{section:chemistry}{{2.2}{4}{Chemical Structure}{subsection.2.2}{}}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces   Coefficients adopted for our chemical network, following \citet  {glover12a}. In this table, $\zeta $ is the cosmic ray primary ionisation rate, $\chi _{\rm  FUV}$ is the normalized FUV radiation field strength, $A_V$ is the visual extinction, $x_{\rm  H} = n_{\rm  H}/n$ is the H abundance, $x_{\rm  H_2} = n_{\rm  H_2}/n$ is the H$_2$ abundance, $T_4 = T/(10^4\tmspace  +\thinmuskip {.1667em}\mathrm  {K})$, \unhbox \voidb@x \hbox {ln($T_e$)}= ln$(8.6173 \times 10^{-5} \times T/\mathrm  {K})$. Note that this network includes several super-species: CH$_x$ agglomerates CH, CH$_2$, etc., and similarly for OH$_x$, and M and M$^+$ agglomerate a number of metallic species with low ionisation potentials (e.g., Fe, Si).}}{5}{table.2}}
\newlabel{table:chemistry}{{2}{5}{Coefficients adopted for our chemical network, following \citet {glover12a}. In this table, $\zeta $ is the cosmic ray primary ionisation rate, $\chi _{\rm FUV}$ is the normalized FUV radiation field strength, $A_V$ is the visual extinction, $x_{\rm H} = n_{\rm H}/n$ is the H abundance, $x_{\rm H_2} = n_{\rm H_2}/n$ is the H$_2$ abundance, $T_4 = T/(10^4\,\mathrm {K})$, \lnte = ln$(8.6173 \times 10^{-5} \times T/\mathrm {K})$. Note that this network includes several super-species: CH$_x$ agglomerates CH, CH$_2$, etc., and similarly for OH$_x$, and M and M$^+$ agglomerate a number of metallic species with low ionisation potentials (e.g., Fe, Si)}{table.2}{}}
\citation{neufeld10a,indriolo12a}
\citation{narayanan12a,narayanan12b}
\citation{papadopoulos10a}
\citation{bisbas15a}
\citation{goldsmith01a}
\citation{osterbrock06a}
\citation{krumholz13a}
\citation{krumholz13a}
\citation{schoier05a}
\citation{launay77a,barinovs05a}
\citation{lique13a,wiesenfeld14a}
\citation{launay77a}
\citation{staemmler91a}
\citation{schroder91a}
\citation{abrahamsson07a}
\citation{jaquet92a}
\citation{yang10a}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3}Thermal State of Clouds}{6}{subsection.2.3}}
\newlabel{ssec:thermal_struct}{{2.3}{6}{Thermal State of Clouds}{subsection.2.3}{}}
\newlabel{equation:goldsmith1}{{11}{6}{Thermal State of Clouds}{equation.11}{}}
\newlabel{equation:goldsmith2}{{12}{6}{Thermal State of Clouds}{equation.11}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4}Statistical Equilibrium}{6}{subsection.2.4}}
\newlabel{section:radiative_transfer}{{2.4}{6}{Statistical Equilibrium}{subsection.2.4}{}}
\newlabel{equation:kmt_stateq}{{13}{6}{Statistical Equilibrium}{equation.13}{}}
\citation{krumholz08a}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.5}Convergence and Computation of the Emergent Luminosity}{7}{subsection.2.5}}
\newlabel{ssec:convergence}{{2.5}{7}{Convergence and Computation of the Emergent Luminosity}{subsection.2.5}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.6}Sample Results}{7}{subsection.2.6}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Results}{7}{section.3}}
\newlabel{section:results}{{3}{7}{Results}{section.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.1}Carbon-based Chemistry}{7}{subsection.3.1}}
\newlabel{section:chemistry_intuition}{{3.1}{7}{Carbon-based Chemistry}{subsection.3.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Physical properties of model clouds inside a galaxy of $M_{\rm  gas} = 10^9$ \unhbox \voidb@x \hbox {M$_{\hbox {$\odot $}}$ }as a function of cloud surface density. These include volume density (top left), chemical abundances (top right), gas kinetic temperature (bottom left), and heating/cooling rates (bottom right). All quantities shown are mass-weighted averages, with the exception that In the gas kinetic temperature panel the different lines correspond to temperatures weighted by H\nobreakspace  {}\textsc  {i} mass, H$_2$ mass, and CO luminosity, respectively. }}{8}{figure.1}}
\newlabel{figure:physical_properties_sd}{{1}{8}{Physical properties of model clouds inside a galaxy of $M_{\rm gas} = 10^9$ \msun as a function of cloud surface density. These include volume density (top left), chemical abundances (top right), gas kinetic temperature (bottom left), and heating/cooling rates (bottom right). All quantities shown are mass-weighted averages, with the exception that In the gas kinetic temperature panel the different lines correspond to temperatures weighted by H~\textsc {i} mass, H$_2$ mass, and CO luminosity, respectively}{figure.1}{}}
\citation{bisbas15a}
\citation{cox11a,debreuck11a,george13a,graciacarpio11a,ivison10a,maiolino05a,rawle13a,stacey10a,swinbank12a,valtchanov11a,venemans12a,wagg12a,wang13a,willott13a,diazsantos15a,schaerer15a,gullberg15a}
\citation{cox11a,debreuck11a,george13a,graciacarpio11a,ivison10a,maiolino05a,rawle13a,stacey10a,swinbank12a,valtchanov11a,venemans12a,wagg12a,wang13a,willott13a,diazsantos15a,schaerer15a,gullberg15a}
\citation{saintonge11a,bothwell13a,casey14a}
\citation{brauher08a}
\citation{diazsantos13a}
\citation{farrah13a}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces $^{12}$CO abundance contours as a function of the volumetric and gas surface densities. Abundance contours are shown for four fiducial star formation rates, which control the far ultraviolet flux and the cosmic ray ionisation rates. At low radiation field strengths/cosmic ray ionisation rates, nearly all of the carbon is in the form of CO. At higher SFRs, UV radiation and cosmic ray ionisations contribute to the destruction of CO, especially at low densities and surface densities. The whitespace in the contour subplots denotes abundances below $10^{-6}$/\unhbox \voidb@x \hbox {H$_2$}. }}{9}{figure.2}}
\newlabel{figure:co_contours}{{2}{9}{$^{12}$CO abundance contours as a function of the volumetric and gas surface densities. Abundance contours are shown for four fiducial star formation rates, which control the far ultraviolet flux and the cosmic ray ionisation rates. At low radiation field strengths/cosmic ray ionisation rates, nearly all of the carbon is in the form of CO. At higher SFRs, UV radiation and cosmic ray ionisations contribute to the destruction of CO, especially at low densities and surface densities. The whitespace in the contour subplots denotes abundances below $10^{-6}$/\htwo }{figure.2}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces Similar to Figure\nobreakspace  {}\ref  {figure:co_contours}, but \unhbox \voidb@x \hbox {\sc  C$^+$}\ abundance contours as a function of gas surface density and volumetric density. \unhbox \voidb@x \hbox {\sc  C$^+$}\ abundances are increased in low volume density and surface density gas, and in high ultraviolet radiation fields and/or cosmic ray fluxes. The whitespace in the contour subplots denotes abundances below $10^{-6}$/\unhbox \voidb@x \hbox {H$_2$}. }}{9}{figure.3}}
\newlabel{figure:cii_contours}{{3}{9}{Similar to Figure~\ref {figure:co_contours}, but \cp \ abundance contours as a function of gas surface density and volumetric density. \cp \ abundances are increased in low volume density and surface density gas, and in high ultraviolet radiation fields and/or cosmic ray fluxes. The whitespace in the contour subplots denotes abundances below $10^{-6}$/\htwo }{figure.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.2}Application to Multiphase Clouds}{9}{subsection.3.2}}
\@writefile{toc}{\contentsline {subsection}{\numberline {3.3}The \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}-FIR Relation}{9}{subsection.3.3}}
\newlabel{section:cii_fir_deficit}{{3.3}{9}{The \cii -FIR Relation}{subsection.3.3}{}}
\citation{narayanan14a}
\citation{graciacarpio11a}
\citation{farrah13a}
\citation{graciacarpio11a}
\citation{farrah13a}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces Radial variation of atomic and molecular abundances in three model clouds in a galaxy of $M_{\rm  gas} = 10^9$ \unhbox \voidb@x \hbox {M$_{\hbox {$\odot $}}$}. The abundances are plotted against the Lagrangian mass enclosed such that a value of M(r)/M$_{\rm  tot}$ = 1 corresponds to the surface of the cloud. Abundances are normalised to their maximum possible value, and plotted as a function of cloud radius. We show three clouds of increasing gas surface density. In general terms, the \unhbox \voidb@x \hbox {H$_2$}\ abundances increase toward the interior of clouds as shielding protects molecules from photodissociation. The carbon transitions from \unhbox \voidb@x \hbox {\sc  C$^+$}\ to CO, with the \unhbox \voidb@x \hbox {\sc  C$^+$}\ predominantly residing in the atomic PDRs and outer shell of \unhbox \voidb@x \hbox {H$_2$}\ gas. Clouds of increasing surface density have an increasing fraction of their gas in molecular \unhbox \voidb@x \hbox {H$_2$}\ form, and increasing fraction of their carbon locked in CO molecules. The oxygen abundances decrease toward the interior of clouds as the atom becomes locked up in CO and, in the inner parts of the highest surface density case, \unhbox \voidb@x \hbox {\sc  OH$_{\rm  x}$}\ molecules. }}{10}{figure.4}}
\newlabel{figure:abundances}{{4}{10}{Radial variation of atomic and molecular abundances in three model clouds in a galaxy of $M_{\rm gas} = 10^9$ \msunend . The abundances are plotted against the Lagrangian mass enclosed such that a value of M(r)/M$_{\rm tot}$ = 1 corresponds to the surface of the cloud. Abundances are normalised to their maximum possible value, and plotted as a function of cloud radius. We show three clouds of increasing gas surface density. In general terms, the \htwo \ abundances increase toward the interior of clouds as shielding protects molecules from photodissociation. The carbon transitions from \cp \ to CO, with the \cp \ predominantly residing in the atomic PDRs and outer shell of \htwo \ gas. Clouds of increasing surface density have an increasing fraction of their gas in molecular \htwo \ form, and increasing fraction of their carbon locked in CO molecules. The oxygen abundances decrease toward the interior of clouds as the atom becomes locked up in CO and, in the inner parts of the highest surface density case, \ohx \ molecules}{figure.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Discussion}{10}{section.4}}
\newlabel{section:discussion}{{4}{10}{Discussion}{section.4}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.1}Calorimetry of Giant Clouds}{10}{subsection.4.1}}
\newlabel{section:calorimetry}{{4.1}{10}{Calorimetry of Giant Clouds}{subsection.4.1}{}}
\citation{graciacarpio11a}
\citation{farrah13a}
\citation{haileydunsheath08a,stacey10a,brisbin15a,gullberg15a,schaerer15a}
\citation{riechers13a,rawle14a,wang13a,capak15a}
\citation{casey14a}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces Theoretical \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}\ luminosities (normalised by the FIR luminosity) as a function of FIR luminosity. The model tracks show predictions for galaxy gas masses log$_{10}$(M$_{\rm  gas}$) = [9,11.3]. The grey points show local \unhbox \voidb@x \hbox {$z\sim $ }0 data, and the red triangles show high-$z$ data. The lowest mass model track corresponds to the left-most one. The \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}-FIR deficit in galaxies owes principally to a decrease in PDR mass in galaxies with increasing infrared luminosity. High-redshift galaxies are observed to be systematically at a higher infrared luminosity at a given \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}/FIR luminosity ratio as compared to low-$z$ galaxies. In our model, this arises because galaxies at high-$z$ have systematically larger gas masses. At a fixed star formation rate, an increased gas mass means lower cloud surface densities on average, which results in higher \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}\ luminosities. High-$z$ detections are from \citet  {cox11a,debreuck11a,george13a,graciacarpio11a,ivison10a,maiolino05a,rawle13a,stacey10a,swinbank12a,valtchanov11a,venemans12a,wagg12a,wang13a,willott13a,diazsantos15a,schaerer15a,gullberg15a}. }}{11}{figure.5}}
\newlabel{figure:cii_fir_masses}{{5}{11}{Theoretical \cii \ luminosities (normalised by the FIR luminosity) as a function of FIR luminosity. The model tracks show predictions for galaxy gas masses log$_{10}$(M$_{\rm gas}$) = [9,11.3]. The grey points show local \zsim 0 data, and the red triangles show high-$z$ data. The lowest mass model track corresponds to the left-most one. The \cii -FIR deficit in galaxies owes principally to a decrease in PDR mass in galaxies with increasing infrared luminosity. High-redshift galaxies are observed to be systematically at a higher infrared luminosity at a given \cii /FIR luminosity ratio as compared to low-$z$ galaxies. In our model, this arises because galaxies at high-$z$ have systematically larger gas masses. At a fixed star formation rate, an increased gas mass means lower cloud surface densities on average, which results in higher \cii \ luminosities. High-$z$ detections are from \citet {cox11a,debreuck11a,george13a,graciacarpio11a,ivison10a,maiolino05a,rawle13a,stacey10a,swinbank12a,valtchanov11a,venemans12a,wagg12a,wang13a,willott13a,diazsantos15a,schaerer15a,gullberg15a}}{figure.5}{}}
\citation{bothwell13a}
\citation{dave10a,geach11a,rodighiero11a,madau14a,narayanan12c,narayanan15a}
\citation{casey14a,ivison11a,simpson15a}
\citation{narayanan15a}
\citation{elbaz11a}
\citation{olsen15a}
\citation{nagamine06a,munoz13a,munoz13b,vallini13a,vallini15a,pallottini15a}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces Cooling rates of individual lines as a function of cloud surface density for a model galaxy of mass $M_{\rm  gas} = 10^9$ \unhbox \voidb@x \hbox {M$_{\hbox {$\odot $}}$}. As the \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}\ luminosities decrease with increasing gas surface density, the principle cooling transitions to CO and \unhbox \voidb@x \hbox {[O\nobreakspace  {}\textsc  {i}}]\ emission lines. At high surface densities, the CO cooling is dominated by high-J rotational transitions. Note, because we only show a subset of the CO lines for clarity, the sum of the cooling rates of the shown CO lines won't add up to the total CO cooling rate shown. }}{12}{figure.6}}
\newlabel{figure:calorimetry}{{6}{12}{Cooling rates of individual lines as a function of cloud surface density for a model galaxy of mass $M_{\rm gas} = 10^9$ \msunend . As the \cii \ luminosities decrease with increasing gas surface density, the principle cooling transitions to CO and \oi \ emission lines. At high surface densities, the CO cooling is dominated by high-J rotational transitions. Note, because we only show a subset of the CO lines for clarity, the sum of the cooling rates of the shown CO lines won't add up to the total CO cooling rate shown}{figure.6}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}/\unhbox \voidb@x \hbox {[O\nobreakspace  {}\textsc  {i}}]\ cooling rates for model compared to data from \citet  {graciacarpio11a} and \citet  {farrah13a}. The \unhbox \voidb@x \hbox {[O\nobreakspace  {}\textsc  {i}}]\ cooling rates are a sum of the $63 \mu $m and $145 \mu $m emission lines. At high gas surface density (or galaxy infrared luminosity), the dominant cooling in the model transitions from \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}\ line emission to \unhbox \voidb@x \hbox {[O\nobreakspace  {}\textsc  {i}}]\ and CO line emission. The orange line shows where the cooling power transitions from \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}\ to \unhbox \voidb@x \hbox {[O\nobreakspace  {}\textsc  {i}}]. }}{12}{figure.7}}
\newlabel{figure:oi_fir}{{7}{12}{\cii /\oi \ cooling rates for model compared to data from \citet {graciacarpio11a} and \citet {farrah13a}. The \oi \ cooling rates are a sum of the $63 \mu $m and $145 \mu $m emission lines. At high gas surface density (or galaxy infrared luminosity), the dominant cooling in the model transitions from \cii \ line emission to \oi \ and CO line emission. The orange line shows where the cooling power transitions from \cii \ to \oi }{figure.7}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.2}Application to High-Redshift Galaxies}{12}{subsection.4.2}}
\newlabel{section:high_redshift}{{4.2}{12}{Application to High-Redshift Galaxies}{subsection.4.2}{}}
\citation{abel09a}
\citation{ferland13a}
\citation{luhman03a}
\citation{pineda14a}
\citation{bisbas15a}
\citation{popping13b}
\citation{munoz15a}
\citation{narayanan11b}
\citation{narayanan11b}
\citation{stacey91a}
\citation{stacey91a}
\citation{diazsantos13a}
\citation{kennicutt12a}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.3}Relationship to other Theoretical Models}{13}{subsection.4.3}}
\newlabel{section:theory}{{4.3}{13}{Relationship to other Theoretical Models}{subsection.4.3}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.4}Relationship to Observations}{13}{subsection.4.4}}
\@writefile{toc}{\contentsline {subsection}{\numberline {4.5}Uncertainties in the Model}{13}{subsection.4.5}}
\newlabel{section:uncertainties}{{4.5}{13}{Uncertainties in the Model}{subsection.4.5}{}}
\citation{kennicutt12a}
\citation{mcall99a,indriolo07a,neufeld10a,wolfire10a}
\citation{abdo10b}
\@writefile{toc}{\contentsline {section}{\numberline {5}Summary}{14}{section.5}}
\newlabel{section:summary}{{5}{14}{Summary}{section.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}/FIR luminosity ratio versus FIR luminosity for our fiducial model (thick blue), and three varying parameters in our cloud models. The example shown is for a $M_{\rm  gas} = 3 \times 10^{9} \unhbox \voidb@x \hbox {M$_{\hbox {$\odot $}}$ }$ galaxy, the average mass (in log-space) of our low-redshift galaxy mass range. See Table\nobreakspace  {}\ref  {table:free_parameters} for variable definitions. }}{14}{figure.8}}
\newlabel{figure:parameter_survey}{{8}{14}{\cii /FIR luminosity ratio versus FIR luminosity for our fiducial model (thick blue), and three varying parameters in our cloud models. The example shown is for a $M_{\rm gas} = 3 \times 10^{9} \msun $ galaxy, the average mass (in log-space) of our low-redshift galaxy mass range. See Table~\ref {table:free_parameters} for variable definitions}{figure.8}{}}
\bibstyle{mnras}
\bibcite{abdo10b}{{1}{2010}{{{Abdo} et~al.}}{{{Abdo} et~al.}}}
\bibcite{abel09a}{{2}{2009}{{{Abel} et~al.}}{{{Abel}, {Dudley}, {Fischer}, {Satyapal} \& {van Hoof}}}}
\bibcite{abrahamsson07a}{{3}{2007}{{{Abrahamsson} et~al.}}{{{Abrahamsson}, {Krems} \& {Dalgarno}}}}
\bibcite{barinovs05a}{{4}{2005}{{{Barinovs} et~al.}}{{{Barinovs}, {van Hemert}, {Krems} \& {Dalgarno}}}}
\bibcite{beirao12a}{{5}{2010}{{{Beir{\~a}o} et~al.}}{{{Beir{\~a}o} et~al.,}}}
\bibcite{bertoldi92a}{{6}{1992}{{{Bertoldi} \& {McKee}}}{{{Bertoldi} \& {McKee}}}}
\bibcite{bigiel08a}{{7}{2008}{{{Bigiel} et~al.}}{{{Bigiel}, {Leroy}, {Walter}, {Brinks}, {de Blok}, {Madore} \& {Thornley}}}}
\bibcite{bisbas15a}{{8}{2015}{{{Bisbas} et~al.}}{{{Bisbas}, {Papadopoulos} \& {Viti}}}}
\bibcite{blanc09a}{{9}{2009}{{{Blanc} et~al.}}{{{Blanc}, {Heiderman}, {Gebhardt}, {Evans} \& {Adams}}}}
\bibcite{bolatto08a}{{10}{2008}{{{Bolatto} et~al.}}{{{Bolatto}, {Leroy}, {Rosolowsky}, {Walter} \& {Blitz}}}}
\bibcite{boselli02a}{{11}{2002}{{{Boselli} et~al.}}{{{Boselli}, {Lequeux} \& {Gavazzi}}}}
\bibcite{bothwell13a}{{12}{2013}{{{Bothwell} et~al.}}{{{Bothwell} et~al.,}}}
\bibcite{brauher08a}{{13}{2008}{{{Brauher} et~al.}}{{{Brauher}, {Dale} \& {Helou}}}}
\bibcite{brisbin15a}{{14}{2015}{{{Brisbin} et~al.}}{{{Brisbin}, {Ferkinhoff}, {Nikola}, {Parshley}, {Stacey}, {Spoon}, {Hailey-Dunsheath} \& {Verma}}}}
\bibcite{capak15a}{{15}{2015}{{{Capak} et~al.}}{{{Capak} et~al.,}}}
\bibcite{casey14a}{{16}{2014}{{{Casey} et~al.}}{{{Casey}, {Narayanan} \& {Cooray}}}}
\bibcite{chomiuk11a}{{17}{2011}{{{Chomiuk} \& {Povich}}}{{{Chomiuk} \& {Povich}}}}
\bibcite{cox11a}{{18}{2011}{{{Cox} et~al.}}{{{Cox} et~al.,}}}
\bibcite{croxall12a}{{19}{2012}{{{Croxall} et~al.}}{{{Croxall} et~al.,}}}
\bibcite{dave10a}{{20}{2010}{{{Dav{\'e}} et~al.}}{{{Dav{\'e}}, {Finlator}, {Oppenheimer}, {Fardal}, {Katz}, {Kere{\v s}} \& {Weinberg}}}}
\bibcite{debreuck11a}{{21}{2011}{{{De Breuck} et~al.}}{{{De Breuck}, {Maiolino}, {Caselli}, {Coppin}, {Hailey-Dunsheath} \& {Nagao}}}}
\bibcite{diazsantos13a}{{22}{2013}{{{D{\'{\i }}az-Santos} et~al.}}{{{D{\'{\i }}az-Santos} et~al.,}}}
\bibcite{diazsantos15a}{{23}{2015}{{{Diaz-Santos} et~al.}}{{{Diaz-Santos} et~al.,}}}
\bibcite{dobbs11a}{{24}{2011}{{{Dobbs} et~al.}}{{{Dobbs}, {Burkert} \& {Pringle}}}}
\bibcite{dobbs13a}{{25}{2013}{{{Dobbs} et~al.}}{{{Dobbs} et~al.,}}}
\bibcite{dobbs14a}{{26}{2014}{{{Dobbs} et~al.}}{{{Dobbs} et~al.,}}}
\bibcite{draine11a}{{27}{2011}{{{Draine}}}{{{Draine}}}}
\bibcite{draine96a}{{28}{1996}{{{Draine} \& {Bertoldi}}}{{{Draine} \& {Bertoldi}}}}
\bibcite{elbaz11a}{{29}{2011}{{{Elbaz} et~al.}}{{{Elbaz} et~al.,}}}
\bibcite{farrah13a}{{30}{2013}{{{Farrah} et~al.}}{{{Farrah} et~al.,}}}
\bibcite{ferland13a}{{31}{2013}{{{Ferland} et~al.}}{{{Ferland} et~al.,}}}
\bibcite{geach11a}{{32}{2011}{{{Geach} et~al.}}{{{Geach}, {Smail}, {Moran}, {MacArthur}, {Lagos} \& {Edge}}}}
\bibcite{george13a}{{33}{2013}{{{George} et~al.}}{{{George} et~al.,}}}
\bibcite{glover12a}{{34}{2012}{{{Glover} \& {Clark}}}{{{Glover} \& {Clark}}}}
\bibcite{glover07a}{{35}{2007}{{{Glover} \& {Mac Low}}}{{{Glover} \& {Mac Low}}}}
\bibcite{glover11a}{{36}{2011}{{{Glover} \& {Mac Low}}}{{{Glover} \& {Mac Low}}}}
\bibcite{goldsmith01a}{{37}{2001}{{{Goldsmith}}}{{{Goldsmith}}}}
\bibcite{goldsmith12a}{{38}{2012}{{{Goldsmith} et~al.}}{{{Goldsmith}, {Langer}, {Pineda} \& {Velusamy}}}}
\bibcite{graciacarpio11a}{{39}{2011}{{{Graci{\'a}-Carpio} et~al.}}{{{Graci{\'a}-Carpio} et~al.,}}}
\bibcite{gullberg15a}{{40}{2015}{{{Gullberg} et~al.}}{{{Gullberg} et~al.,}}}
\bibcite{haileydunsheath08a}{{41}{2008}{{{Hailey-Dunsheath} et~al.}}{{{Hailey-Dunsheath}, {Nikola}, {Oberst}, {Parshley}, {Stacey}, {Farrah}, {Benford} \& {Staguhn}}}}
\bibcite{herreracamus15a}{{42}{2015}{{{Herrera-Camus} et~al.}}{{{Herrera-Camus} et~al.,}}}
\bibcite{heyer15a}{{43}{2015}{{{Heyer} \& {Dame}}}{{{Heyer} \& {Dame}}}}
\bibcite{indriolo07a}{{44}{2007}{{{Indriolo} et~al.}}{{{Indriolo}, {Geballe}, {Oka} \& {McCall}}}}
\bibcite{indriolo12a}{{45}{2012}{{{Indriolo} et~al.}}{{{Indriolo}, {Neufeld}, {Gerin}, {Geballe}, {Black}, {Menten} \& {Goicoechea}}}}
\bibcite{iono06a}{{46}{2006}{{{Iono} et~al.}}{{{Iono} et~al.,}}}
\bibcite{ivison10a}{{47}{2010}{{{Ivison} et~al.}}{{{Ivison} et~al.,}}}
\bibcite{ivison11a}{{48}{2011}{{{Ivison} et~al.}}{{{Ivison}, {Papadopoulos}, {Smail}, {Greve}, {Thomson}, {Xilouris} \& {Chapman}}}}
\bibcite{jaquet92a}{{49}{1992}{{{Jaquet} et~al.}}{{{Jaquet}, {Staemmler}, {Smith} \& {Flower}}}}
\bibcite{kennicutt12a}{{50}{2012}{{{Kennicutt} \& {Evans}}}{{{Kennicutt} \& {Evans}}}}
\bibcite{krumholz12c}{{51}{2012}{{{Krumholz}}}{{{Krumholz}}}}
\bibcite{krumholz13a}{{52}{2013a}{{{Krumholz}}}{{{Krumholz}}}}
\bibcite{krumholz13c}{{53}{2013b}{{{Krumholz}}}{{{Krumholz}}}}
\bibcite{krumholz14a}{{54}{2014}{{{Krumholz}}}{{{Krumholz}}}}
\bibcite{krumholz07b}{{55}{2007}{{{Krumholz} \& {Tan}}}{{{Krumholz} \& {Tan}}}}
\bibcite{krumholz08a}{{56}{2008}{{{Krumholz} et~al.}}{{{Krumholz}, {McKee} \& {Tumlinson}}}}
\bibcite{krumholz09a}{{57}{2009a}{{{Krumholz} et~al.}}{{{Krumholz}, {McKee} \& {Tumlinson}}}}
\bibcite{krumholz09b}{{58}{2009b}{{{Krumholz} et~al.}}{{{Krumholz}, {McKee} \& {Tumlinson}}}}
\@writefile{lof}{\contentsline {figure}{\numberline {A1}{\ignorespaces Convergence test for number of radial zones in model clouds. Test shows model \unhbox \voidb@x \hbox {\sc  [C\nobreakspace  {}\textsc  {ii}]}-FIR deficit for a galaxy of mass $M_{\rm  gas} = 3 \times 10^9$ \unhbox \voidb@x \hbox {M$_{\hbox {$\odot $}}$ }, the average mass (in log-space) of our low-redshift galaxy mass range. }}{15}{figure.A1.1}}
\newlabel{figure:convergence}{{A1}{15}{Convergence test for number of radial zones in model clouds. Test shows model \cii -FIR deficit for a galaxy of mass $M_{\rm gas} = 3 \times 10^9$ \msun , the average mass (in log-space) of our low-redshift galaxy mass range}{figure.A1.1}{}}
\@writefile{toc}{\contentsline {section}{\numberline {A}Resolution Tests}{15}{section.A1}}
\newlabel{section:resolution}{{A}{15}{Resolution Tests}{section.A1}{}}
\bibcite{krumholz11a}{{59}{2011}{{{Krumholz} et~al.}}{{{Krumholz}, {Leroy} \& {McKee}}}}
\bibcite{krumholz12a}{{60}{2012}{{{Krumholz} et~al.}}{{{Krumholz}, {Dekel} \& {McKee}}}}
\bibcite{launay77a}{{61}{1977}{{{Launay} \& {Roueff}}}{{{Launay} \& {Roueff}}}}
\bibcite{leech99a}{{62}{1999}{{{Leech} et~al.}}{{{Leech} et~al.,}}}
\bibcite{leroy13a}{{63}{2013}{{{Leroy} et~al.}}{{{Leroy} et~al.,}}}
\bibcite{lique13a}{{64}{2013}{{{Lique} et~al.}}{{{Lique}, {Werfelli}, {Halvick}, {Stoecklin}, {Faure}, {Wiesenfeld} \& {Dagdigian}}}}
\bibcite{luhman98a}{{65}{1998}{{{Luhman} et~al.}}{{{Luhman} et~al.,}}}
\bibcite{luhman03a}{{66}{2003a}{{{Luhman} et~al.}}{{{Luhman}, {Brice{\~n}o}, {Stauffer}, {Hartmann}, {Barrado y Navascu{\'e}s} \& {Caldwell}}}}
\bibcite{luhman03b}{{67}{2003b}{{{Luhman} et~al.}}{{{Luhman}, {Satyapal}, {Fischer}, {Wolfire}, {Sturm}, {Dudley}, {Lutz} \& {Genzel}}}}
\bibcite{madau14a}{{68}{2014}{{{Madau} \& {Dickinson}}}{{{Madau} \& {Dickinson}}}}
\bibcite{maiolino05a}{{69}{2005}{{{Maiolino} et~al.}}{{{Maiolino} et~al.,}}}
\bibcite{malhotra97a}{{70}{1997}{{{Malhotra} et~al.}}{{{Malhotra} et~al.,}}}
\bibcite{malhotra01a}{{71}{2001}{{{Malhotra} et~al.}}{{{Malhotra} et~al.,}}}
\bibcite{mcall99a}{{72}{1999}{{{McCall} et~al.}}{{{McCall}, {Geballe}, {Hinkle} \& {Oka}}}}
\bibcite{mckee10a}{{73}{2010}{{{McKee} \& {Krumholz}}}{{{McKee} \& {Krumholz}}}}
\bibcite{munoz13b}{{74}{2013a}{{{Mu{\~n}oz} \& {Furlanetto}}}{{{Mu{\~n}oz} \& {Furlanetto}}}}
\bibcite{munoz13a}{{75}{2013b}{{{Mu{\~n}oz} \& {Furlanetto}}}{{{Mu{\~n}oz} \& {Furlanetto}}}}
\bibcite{munoz15a}{{76}{2015}{{{Mu{\~n}oz} \& {Oh}}}{{{Mu{\~n}oz} \& {Oh}}}}
\bibcite{murphy11a}{{77}{2011}{{{Murphy} et~al.}}{{{Murphy} et~al.,}}}
\bibcite{nagamine06a}{{78}{2006}{{{Nagamine} et~al.}}{{{Nagamine}, {Wolfe} \& {Hernquist}}}}
\bibcite{narayanan12b}{{79}{2012}{{{Narayanan} \& {Dav{\'e}}}}{{{Narayanan} \& {Dav{\'e}}}}}
\bibcite{narayanan14a}{{80}{2014}{{{Narayanan} \& {Krumholz}}}{{{Narayanan} \& {Krumholz}}}}
\bibcite{narayanan11a}{{81}{2011a}{{{Narayanan} et~al.}}{{{Narayanan}, {Cox}, {Hayward} \& {Hernquist}}}}
\bibcite{narayanan11b}{{82}{2011b}{{{Narayanan} et~al.}}{{{Narayanan}, {Krumholz}, {Ostriker} \& {Hernquist}}}}
\bibcite{narayanan12a}{{83}{2012a}{{{Narayanan} et~al.}}{{{Narayanan}, {Krumholz}, {Ostriker} \& {Hernquist}}}}
\bibcite{narayanan12c}{{84}{2012b}{{{Narayanan} et~al.}}{{{Narayanan}, {Bothwell} \& {Dav{\'e}}}}}
\bibcite{narayanan15a}{{85}{2015}{{{Narayanan} et~al.}}{{{Narayanan} et~al.,}}}
\bibcite{nelson99a}{{86}{1999}{{{Nelson} \& {Langer}}}{{{Nelson} \& {Langer}}}}
\bibcite{neufeld10a}{{87}{2010}{{{Neufeld} et~al.}}{{{Neufeld} et~al.,}}}
\bibcite{nikola98a}{{88}{1998}{{{Nikola} et~al.}}{{{Nikola}, {Genzel}, {Herrmann}, {Madden}, {Poglitsch}, {Geis}, {Townes} \& {Stacey}}}}
\bibcite{olsen15a}{{89}{2015}{{{Olsen} et~al.}}{{{Olsen}, {Greve}, {Narayanan}, {Thompson}, {Toft} \& {Brinch}}}}
\bibcite{osterbrock06a}{{90}{2006}{{{Osterbrock} \& {Ferland}}}{{{Osterbrock} \& {Ferland}}}}
\bibcite{pallottini15a}{{91}{2015}{{{Pallottini} et~al.}}{{{Pallottini}, {Gallerani}, {Ferrara}, {Yue}, {Vallini}, {Maiolino} \& {Feruglio}}}}
\bibcite{papadopoulos10a}{{92}{2010}{{{Papadopoulos}}}{{{Papadopoulos}}}}
\bibcite{pineda14a}{{93}{2014}{{{Pineda} et~al.}}{{{Pineda}, {Langer} \& {Goldsmith}}}}
\bibcite{popping13b}{{94}{2013}{{{Popping} et~al.}}{{{Popping}, {P{\'e}rez-Beaupuits}, {Spaans}, {Trager} \& {Somerville}}}}
\bibcite{rawle13a}{{95}{2013}{{{Rawle} et~al.}}{{{Rawle} et~al.,}}}
\bibcite{rawle14a}{{96}{2014}{{{Rawle} et~al.}}{{{Rawle} et~al.,}}}
\bibcite{riechers13a}{{97}{2013}{{{Riechers} et~al.}}{{{Riechers} et~al.}}}
\bibcite{rigopoulou14a}{{98}{2014}{{{Rigopoulou} et~al.}}{{{Rigopoulou} et~al.,}}}
\bibcite{robitaille10a}{{99}{2010}{{{Robitaille} \& {Whitney}}}{{{Robitaille} \& {Whitney}}}}
\bibcite{rodighiero11a}{{100}{2011}{{{Rodighiero} et~al.}}{{{Rodighiero} et~al.}}}
\bibcite{saintonge11a}{{101}{2011}{{{Saintonge} et~al.}}{{{Saintonge} et~al.,}}}
\bibcite{sargsyan12a}{{102}{2012}{{{Sargsyan} et~al.}}{{{Sargsyan} et~al.,}}}
\bibcite{schaerer15a}{{103}{2015}{{{Schaerer} et~al.}}{{{Schaerer} et~al.,}}}
\bibcite{schoier05a}{{104}{2005}{{{Sch{\"o}ier} et~al.}}{{{Sch{\"o}ier}, {van der Tak}, {van Dishoeck} \& {Black}}}}
\bibcite{schroder91a}{{105}{1991}{{{Schroder} et~al.}}{{{Schroder}, {Staemmler}, {Smith}, {Flower} \& {Jaquet}}}}
\bibcite{shetty13b}{{106}{2013a}{{{Shetty} et~al.}}{{{Shetty}, {Kelly}, {Rahman}, {Bigiel}, {Bolatto}, {Clark}, {Klessen} \& {Konstandin}}}}
\bibcite{shetty13a}{{107}{2013b}{{{Shetty} et~al.}}{{{Shetty}, {Kelly} \& {Bigiel}}}}
\bibcite{simpson15a}{{108}{2015}{{{Simpson} et~al.}}{{{Simpson} et~al.,}}}
\bibcite{stacey91a}{{109}{1991}{{{Stacey} et~al.}}{{{Stacey}, {Geis}, {Genzel}, {Lugten}, {Poglitsch}, {Sternberg} \& {Townes}}}}
\bibcite{stacey10a}{{110}{2010}{{{Stacey} et~al.}}{{{Stacey}, {Hailey-Dunsheath}, {Ferkinhoff}, {Nikola}, {Parshley}, {Benford}, {Staguhn} \& {Fiolet}}}}
\bibcite{staemmler91a}{{111}{1991}{{{Staemmler} \& {Flower}}}{{{Staemmler} \& {Flower}}}}
\bibcite{swinbank12a}{{112}{2012}{{{Swinbank} et~al.}}{{{Swinbank} et~al.,}}}
\bibcite{vallini13a}{{113}{2013}{{{Vallini} et~al.}}{{{Vallini}, {Gallerani}, {Ferrara} \& {Baek}}}}
\bibcite{vallini15a}{{114}{2015}{{{Vallini} et~al.}}{{{Vallini}, {Gallerani}, {Ferrara}, {Pallottini} \& {Yue}}}}
\bibcite{valtchanov11a}{{115}{2011}{{{Valtchanov} et~al.}}{{{Valtchanov} et~al.,}}}
\bibcite{venemans12a}{{116}{2012}{{{Venemans} et~al.}}{{{Venemans} et~al.,}}}
\bibcite{wagg12a}{{117}{2012}{{{Wagg} et~al.}}{{{Wagg} et~al.,}}}
\bibcite{wang13a}{{118}{2013}{{{Wang} et~al.}}{{{Wang} et~al.,}}}
\bibcite{wiesenfeld14a}{{119}{2014}{{{Wiesenfeld} \& {Goldsmith}}}{{{Wiesenfeld} \& {Goldsmith}}}}
\bibcite{willott13a}{{120}{2013}{{{Willott} et~al.}}{{{Willott}, {Omont} \& {Bergeron}}}}
\bibcite{wolfire03a}{{121}{2003}{{{Wolfire} et~al.}}{{{Wolfire}, {McKee}, {Hollenbach} \& {Tielens}}}}
\bibcite{wolfire10a}{{122}{2010}{{{Wolfire} et~al.}}{{{Wolfire}, {Hollenbach} \& {McKee}}}}
\bibcite{yang10a}{{123}{2010}{{{Yang} et~al.}}{{{Yang}, {Stancil}, {Balakrishnan} \& {Forrey}}}}
\bibcite{delooze11a}{{124}{2011}{{{de Looze} et~al.}}{{{de Looze}, {Baes}, {Bendo}, {Cortese} \& {Fritz}}}}
\bibcite{vandishoeck88a}{{125}{1988}{{{van Dishoeck} \& {Black}}}{{{van Dishoeck} \& {Black}}}}


==> x.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\citation{malhotra97a,luhman98a,nikola98a}
\citation{stacey91a}
\citation{goldsmith12a}
\citation{stacey91a}
\citation{leech99a}
\citation{boselli02a}
\citation{delooze11a,sargsyan12a,pineda14a,herreracamus15a}
\citation{olsen15a}
\newlabel{firstpage}{{}{1}{}{Doc-Start}{}}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}}
\newlabel{section:introduction}{{1}{1}{Introduction}{section.1}{}}
\citation{malhotra97a,malhotra01a,luhman98a,luhman03b}
\citation{graciacarpio11a}
\citation{diazsantos13a}
\citation{beirao12a}
\citation{croxall12a}
\citation{farrah13a}
\citation{casey14a}
\citation{iono06a,stacey10a,wagg12a,swinbank12a,rawle13a,riechers13a,wang13a,rigopoulou14a,brisbin15a}
\citation{krumholz08a,krumholz09a,mckee10a}
\citation{krumholz13a,krumholz13c}
\citation{krumholz08a,krumholz09a,krumholz09b}
\citation{mckee10a}
\@writefile{toc}{\contentsline {section}{\numberline {2}Model Description}{2}{section.2}}
\newlabel{section:model}{{2}{2}{Model Description}{section.2}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.1}Cloud Physical Structure}{2}{subsection.2.1}}
\newlabel{ssec:phys_struct}{{2.1}{2}{Cloud Physical Structure}{subsection.2.1}{}}
\newlabel{equation:kmt}{{1}{2}{Cloud Physical Structure}{equation.1}{}}
\citation{bertoldi92a}
\citation{dobbs11a,dobbs13a,heyer15a}
\citation{krumholz11a,glover11a,krumholz12c}
\citation{krumholz07b,krumholz12a,krumholz14a}
\citation{dobbs14a,heyer15a}
\citation{kennicutt12a}
\citation{bigiel08a,blanc09a,narayanan11a,narayanan11b,narayanan12a,shetty13b,shetty13a}
\citation{narayanan12a}
\@writefile{lot}{\contentsline {table}{\numberline {1}{\ignorespaces Parameters used in cloud models  }}{3}{table.1}}
\newlabel{table:free_parameters}{{1}{3}{Parameters used in cloud models}{table.1}{}}
\newlabel{equation:mass}{{3}{3}{Cloud Physical Structure}{equation.3}{}}
\newlabel{eq:sigmac}{{6}{3}{Cloud Physical Structure}{equation.6}{}}
\newlabel{eq:sfr}{{7}{3}{Cloud Physical Structure}{equation.7}{}}
\newlabel{eq:tff}{{8}{3}{Cloud Physical Structure}{equation.8}{}}
\citation{wolfire03a}
\citation{heyer15a}
\citation{robitaille10a}
\citation{chomiuk11a}
\citation{bolatto08a,leroy13a}
\citation{saintonge11a,bothwell13a}
\citation{murphy11a}
\citation{kennicutt12a}
\citation{draine11a}
\citation{nelson99a}
\citation{glover07a}
\citation{glover07a}
\citation{glover12a}
\citation{glover12a}
\citation{glover12a}
\citation{glover12a}
\citation{robitaille10a,chomiuk11a}
\citation{glover12a}
\citation{draine96a}
\citation{vandishoeck88a}
\newlabel{eq:rhoscaling}{{9}{4}{Cloud Physical Structure}{equation.9}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.2}Chemical Structure}{4}{subsection.2.2}}
\newlabel{section:chemistry}{{2.2}{4}{Chemical Structure}{subsection.2.2}{}}
\@writefile{lot}{\contentsline {table}{\numberline {2}{\ignorespaces   Coefficients adopted for our chemical network, following \citet  {glover12a}. In this table, $\zeta $ is the cosmic ray primary ionisation rate, $\chi _{\rm  FUV}$ is the normalized FUV radiation field strength, $A_V$ is the visual extinction, $x_{\rm  H} = n_{\rm  H}/n$ is the H abundance, $x_{\rm  H_2} = n_{\rm  H_2}/n$ is the H$_2$ abundance, $T_4 = T/(10^4\tmspace  +\thinmuskip {.1667em}\mathrm  {K})$, \unhbox \voidb@x \hbox {ln($T_e$)}= ln$(8.6173 \times 10^{-5} \times T/\mathrm  {K})$. Note that this network includes several super-species: CH$_x$ agglomerates CH, CH$_2$, etc., and similarly for OH$_x$, and M and M$^+$ agglomerate a number of metallic species with low ionisation potentials (e.g., Fe, Si).}}{5}{table.2}}
\newlabel{table:chemistry}{{2}{5}{Coefficients adopted for our chemical network, following \citet {glover12a}. In this table, $\zeta $ is the cosmic ray primary ionisation rate, $\chi _{\rm FUV}$ is the normalized FUV radiation field strength, $A_V$ is the visual extinction, $x_{\rm H} = n_{\rm H}/n$ is the H abundance, $x_{\rm H_2} = n_{\rm H_2}/n$ is the H$_2$ abundance, $T_4 = T/(10^4\,\mathrm {K})$, \lnte = ln$(8.6173 \times 10^{-5} \times T/\mathrm {K})$. Note that this network includes several super-species: CH$_x$ agglomerates CH, CH$_2$, etc., and similarly for OH$_x$, and M and M$^+$ agglomerate a number of metallic species with low ionisation potentials (e.g., Fe, Si)}{table.2}{}}
\citation{neufeld10a,indriolo12a}
\citation{narayanan12a,narayanan12b}
\citation{papadopoulos10a}
\citation{bisbas15a}
\citation{goldsmith01a}
\citation{osterbrock06a}
\citation{krumholz13a}
\citation{krumholz13a}
\citation{schoier05a}
\citation{launay77a,barinovs05a}
\citation{lique13a,wiesenfeld14a}
\citation{launay77a}
\citation{staemmler91a}
\citation{schroder91a}
\citation{abrahamsson07a}
\citation{jaquet92a}
\citation{yang10a}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.3}Thermal State of Clouds}{6}{subsection.2.3}}
\newlabel{ssec:thermal_struct}{{2.3}{6}{Thermal State of Clouds}{subsection.2.3}{}}
\newlabel{equation:goldsmith1}{{11}{6}{Thermal State of Clouds}{equation.11}{}}
\newlabel{equation:goldsmith2}{{12}{6}{Thermal State of Clouds}{equation.11}{}}
\@writefile{toc}{\contentsline {subsection}{\numberline {2.4}Statistical Equilibrium}{6}{subsection.2.4}}
\newlabel{section:radiative_transfer}{{2.4}{6}{Statistical Equilibrium}{subsection.2.4}{}}
\newlabel{equation:kmt_stateq}{{13}{6}{Statistical Equilibrium}{equation.13}{}}
\citation{krumholz08a}

